Exploring Data Pipelines through the Process Lens: a Reference Model forComputer Vision

Researchers have identified datasets used for training computer vision (CV) models as an important source of hazardous outcomes, and continue to examine popular CV datasets to expose their harms. These works tend to treat datasets as objects, or focus on particular steps in data production pipelines. We argue here that we could further systematize our analysis of harms by examining CV data pipelines through a process-oriented lens that captures the creation, the evolution and use of these datasets. As a step towards cultivating a process-oriented lens, we embarked on an empirical study of CV data pipelines informed by the field of method engineering. We present here a preliminary result: a reference model of CV data pipelines. Besides exploring the questions that this endeavor raises, we discuss how the process lens could support researchers in discovering understudied issues, and could help practitioners in making their processes more transparent.

==> other_propositions.tex <==
%%%%%%%%% BODY TEXT
 \agathe{From what we discussed yesterday, I arrived at more or less three possible papers / with some overlapping messages but possibly in different levels of details. -> which one do you think would be best to start with? }
 \agathe{I'm not sure whether that would be "smart" to choose like this, but maybe we should start with the closest to GJ's idea of computer science? -- which might be the third proposition, the most empirical one}
 \agathe{Or generally, I wonder how to envision workshop papers presenting works that are later extended as full paper. Should the points be the same but extended? or should we use one of the angles of discussion here for the workshop, and one of the other angles for a full paper?}


\section{Proposition 1}
The theory one could focus on:

- why representation is not the issue, but operational data (that will be very controversial for this community, but if we pull it off, it will be a hit)

- a subpoint could be the play with human-centricity and how the same pipelines are used for other types of foundations 

- and that these things in totality cannot be resolved through a representational approach but requires a bigger discussion

\section{Proposition 2}

*** Intro
We note that CV research does not necessarily encourage multidisiplinary works, works on data, and HCI-oriented works around computer vision. We question how such works could look like. 
We propose to adopt new multidisciplinary approaches for investigating computer vision research and practices around "ethics".
In this paper, we give an overview of these approaches, and we discuss the first new insights that these approaches brought us. These insights span a broad range of topics, from how pure CS researchers create datasets and report on them, to how interdisciplinary researchers orient their focus of research and the methods they rely on or propose.


*** The new approaches we propose

1) First approach: build a clear reference (and modular) pipeline through systematic surveys and interviews.

2) Then, comparative approaches:
\begin{itemize}
    \item   look at dataset papers from different time periods -> to udnerstand how the focuses/interests evolved, and how the pipelines evolved with them.
    \item  survey reference data pipelines and interviews, along what is mentioned in papers and what is left implicit (hyperprameters, activities, reasoning behind choices of parameters, metrics)  -> to understand what are the priorities and main focuses of researchers and practitioners, and what is left out, or unknown.

    \item  look at applications and more "theoretical"? research through interviews and paper surveys -> to understand whether the object of study is actually the same, or to identify potential gaps between research and pipelines used in practice.
    
    \item look at harms mentioned in cv and non-computer vision literature and map/adapt them to the reference pipeline -> to identify harms not previously investigated in the computer vision context, and to have an ordered list.
    % \item  method: study rigor of data pipelines using experiments evaluating metrics used in different activities -> to "validate" the harms

    \item  compare these harms extracted from CS, social science and "art" literature  -> to understand which harms receive much interests (it might also indicate some influences from different actors of computer vision field).
    \item  look at humans and non-humans pipelines, metrics to understand what is going on with computer vision -> to understand strength of the work on human harms?
    
\end{itemize}


*** The insights we get

\begin{itemize}
    \item Critical works around computer vision: focus on representation and not operationalization, lack of systematic list of impact of pipelines on "ethical issues"
    \item CV researcher's practices: 1)  lack of reporting on certain activities, choices; 2) creation or use of large datasets , not necessarily reflecting other industry needs
    \item Awareness of 'ethical issues': assumptions about choices, that might not be correct, or that might trade-off with "ethical" issues --while not being aware of it.
\end{itemize}


\section{Proposition 3}

*** Empirical work

As stated in the call for paper, CV is facing a transparency problem. We believe this problem is not just relevant for being able to understand how models are built in general, but also because it betrays a lack of awareness from researchers and practitioners on the impact that the choices they make for their pipelines have on populations possibly affected by the models.

In this paper, we strive for creating a clear framework that could be further used to support transparency efforts, especially in relation to "ethical" issues.

For that, we first create a reference model of the computer vision pipelines.
We then identify as exhaustively as possible? "ethical issues" that can apply to the pipelines and map them onto specific elements of these pipelines. This forms a framework that should support further transparency efforts as it shows clear elements of the pipelines that should be reported on, and reflected on when creating the pipelines.

*** Method:
Challenges in doing so are the following:
a) creating a reference model that is representative of diverse CV applications (For usability) while each application might be using different pipelines;
b) creating s reference model that reflects accurately the pipelines while papers do not actually report all their activities, parameters, reasoning, etc;
c) creating a reference model that is specific enough to allow  reporting of precise enough elements for understanding/foreseeing ethical issues;
d) identifying and mapping a complete enough? set of "ethical" issues that can arise from the pipelines.

How we tackle these challenges: 
a) we perform a systematic survey of CV literature
b) we complete it with interviews from industry, and from application papers that use CV.
c) we survey ethical issues/harms mentioned in broader CS literature, interdisciplinary works, and other fields, and map them to the pipelines.

*** Results:
We present our model of the pipelines.
We present our mapping.

*** Discussion - > would we have space for some discussion?
e.g. about what the different communities deem important or not to report, to investigate as ethical issues, etc.

*** Future work:
perform the interviews to complete the reference model and to understand how aware practitioners are of the issues, etc.; perform experiments to "prove" some of the harms.
